Energy-based Out-of-distribution Detection

Determining whether inputs are out-of-distribution (OOD) is an essential building block for safely deploying machine learning models in the open world. However, previous methods relying on the softmax confidence score suffer from overconfident posterior distributions for OOD data. We propose a unified framework for OOD detection that uses an energy score. We show that energy scores better distinguish in- and out-of-distribution samples than the traditional approach using the softmax scores. Unlike softmax confidence scores, energy scores are theoretically aligned with the probability density of the inputs and are less susceptible to the overconfidence issue. Within this framework, energy can be flexibly used as a scoring function for any pre-trained neural classifier as well as a trainable cost function to shape the energy surface explicitly for OOD detection. On a CIFAR-10 pre-trained WideResNet, using the energy score reduces the average FPR (at TPR 95%) by 18.03% compared to the softmax confidence score. With energy-based training, our method outperforms the state-of-the-art on common benchmarks.

==> tables/wrn_allconv.tex <==
\begin{table*}[]
        \begin{adjustbox}{width=\columnwidth,center}
                \begin{tabular}{ll|ccc|ccc}
                        \toprule
             \multirow{4}{0.06\linewidth}{\textbf{Dataset $\mathcal{D}_{\text{out}}^{\text{test}}$}}  & &\textbf{FPR}  &  \textbf{AUROC}  & \textbf{AUPR}  &\textbf{FPR}  & \textbf{AUROC}    &\textbf{AUPR}   \\
                 & &  $\textbf{(95\% TPR)}$ & $\textbf{}$  & & $\textbf{(95\% TPR)}$ & $\textbf{}$  \\
                        & & $\downarrow$ & $\uparrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\uparrow$ \\ \cline{3-8}
                        & & \multicolumn{3}{c|}{\textbf{WRN}} & \multicolumn{3}{c}{\textbf{ Allconv}} \\  \hline
                        \multirow{5}{0.06\linewidth}{{\textbf{Texture}}}
                        & Softmax score \cite{hendrycks2016baseline} & 59.28 & 88.50 & 97.16 & 54.18 & 90.81 & 97.99 \\
                        & Energy score (ours) & 52.79 & 85.22 & 95.41 & 39.66 & 91.89 & 98.07\\
                        & ODIN \cite{liang2018enhancing} & 49.12 & 84.97 & 95.28 & 35.34 & 92.39 & 98.17  \\%(T=10, noise=0.0004/0.0024)
                        & Mahalanobis \cite{lee2018simple} & 15.00 & 97.33 & 99.41 & 61.31 & 80.23 & 94.73  \\
                        & OE \cite{hendrycks2018deep} & 12.94 & 97.73 & 99.52 & 18.43 & 96.79 & 99.30 \\
                        & Energy fine-tuning (ours) & 5.34 & 98.56 & 99.68 & 6.17 & 98.73 & 99.74\\
                        \hline
                        %------------------------SVHN----------------------
                        \multirow{5}{0.06\linewidth}{{\textbf{SVHN}}}
                        & Softmax score \cite{hendrycks2016baseline} & 48.49 & 91.89 & 98.27 & 54.37 & 92.79 & 98.59\\
                        & Energy score (ours) & 35.59 & 90.96 & 97.64 & 32.03 & 95.41 & 99.11\\
                        & ODIN \cite{liang2018enhancing} & 33.55 & 91.96 & 98.00 & 14.31 & 97.43 & 99.46 \\
                        & Mahalanobis \cite{lee2018simple} & 12.89 & 97.62 & 99.47 & 37.32 & 91.80 & 98.11 \\
                        & OE \cite{hendrycks2018deep} & 4.36 & 98.63 & 99.74 & 8.51 & 98.49 & 99.70\\
                        & Energy fine-tuning (ours) & 1.04 & 99.41 & 99.89 & 2.14 & 99.31 & 99.87\\
                        \hline
                        % ----------------------- Places365 -------------
                        \multirow{5}{0.06\linewidth}{{\textbf{ Places365}}}
                        & Softmax score \cite{hendrycks2016baseline} & 59.48 & 88.20 & 97.10 & 63.67 & 87.87 & 97.25\\
                        & Energy score (ours) & 40.14 & 89.89 & 97.30 & 42.95 & 91.40 & 97.96\\
                        & ODIN \cite{liang2018enhancing} & 57.40 & 84.49 & 95.82 & 46.42 & 90.81 & 97.89\\
                        & Mahalanobis \cite{lee2018simple} & 68.57 & 84.61 & 96.20 & 95.52 & 58.78 & 88.68 \\
                        & OE \cite{hendrycks2018deep} & 19.07 & 96.16 & 99.06 & 26.85 & 94.78 & 98.78\\
                        & Energy fine-tuning (ours) & 9.00 & 97.48 & 99.35 & 12.06 & 97.08 & 99.29\\
                        \hline
                        % ----------------------- LSUN-C -----------------
                        \multirow{5}{0.06\linewidth}{{\textbf{ LSUN-C}}}
                        & Softmax score \cite{hendrycks2016baseline} & 30.80 & 95.65 & 99.13 & 26.02 & 96.47 & 99.30\\
                        & Energy score (ours) & 8.26 & 98.35 & 99.66 & 3.65 & 99.25 & 99.85\\
                        & ODIN \cite{liang2018enhancing} & 15.52 & 97.04 & 99.33 & 2.30 & 99.46 & 99.89\\
                        &  Mahalanobis \cite{lee2018simple} & 39.22 & 94.15 & 98.81 & 82.54 & 64.48 & 89.72\\
                        & OE \cite{hendrycks2018deep} & 2.89 & 99.49 & 99.90 & 3.58 & 99.32 & 99.86\\
                        & Energy fine-tuning (ours) & 1.67 & 99.32 & 99.86 & 1.34 & 99.49 & 99.90\\
                        \hline
                        % --------------------LSUN-R --------------------
                        \multirow{5}{0.06\linewidth}{{\textbf{ LSUN Resize}}}
                        & Softmax score \cite{hendrycks2016baseline} & 52.15 & 91.37 & 98.12 & 54.40 & 91.78 & 98.34\\
                        & Energy score (ours) & 27.58 & 94.24 & 98.67 & 21.31 & 96.57 & 99.31\\
                        & ODIN \cite{liang2018enhancing} & 26.62 & 94.57 & 98.77 & 13.79 & 97.60 & 99.52\\
                        & Mahalanobis \cite{lee2018simple} & 42.62 & 93.23 & 98.60 & 94.92 & 66.15 & 91.56\\
                        & OE \cite{hendrycks2018deep} & 5.59 & 98.94 & 99.79 & 11.89 & 98.05 & 99.61\\
                        & Energy fine-tuning (ours) & 1.25 & 99.39 & 99.88  & 3.85 & 98.92 & 99.79\\
                        \hline
                        % -------------iSUN --------------------
                        \multirow{5}{0.06\linewidth}{{\textbf{iSUN}}}
                        & Softmax score \cite{hendrycks2016baseline} & 56.03 & 89.83 & 97.74 & 54.02 & 91.96 & 98.38\\
                        & Energy score (ours) & 33.68 & 92.62 & 98.27 & 19.98 & 96.78 & 99.36\\
                        & ODIN \cite{liang2018enhancing} & 32.05 & 93.50 & 98.54 & 13.96 & 97.66 & 99.53\\
                        & Mahalanobis \cite{lee2018simple} & 44.18 & 92.66 & 98.45 & 94.62 & 65.33 & 91.17\\
                        & OE \cite{hendrycks2018deep} & 6.32 & 98.85 & 99.77 & 13.20 & 97.75 & 99.54\\
                        & Energy fine-tuning (ours) & 1.60 & 99.33 & 99.87 & 3.86 & 98.89 & 99.78 \\
                        %& EG fine-tuning $E_F,T=10$ (ours) \\
                        \bottomrule
                \end{tabular}
        \end{adjustbox}
        \vspace{-0.2cm}
        \caption[]{\small OOD Detection performance of CIFAR-10 as in-distribution for each OOD test dataset.
        The Mahalanobis score is calculated using the features of the second-to-last layer.}
        \label{tab:cifar10-results}
\end{table*}



\begin{table*}[]
        \begin{adjustbox}{width=\columnwidth,center}
                \begin{tabular}{ll|ccc|ccc}
                        \toprule
       \multirow{4}{0.06\linewidth}{\textbf{Dataset $\mathcal{D}_{\text{out}}^{\text{test}}$}}  & &\textbf{FPR}  &  \textbf{ AUROC}  & \textbf{ AUPR}  &\textbf{FPR}  & \textbf{AUROC}  &\textbf{AUPR}   \\
                 & &  $\textbf{(95\% TPR)}$ & $\textbf{}$  & & $\textbf{(95\% TPR)}$ & $\textbf{}$  \\
                        & & $\downarrow$ & $\uparrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\uparrow$ \\ \cline{3-8}
                        & & \multicolumn{3}{c|}{\textbf{WRN}} & \multicolumn{3}{c}{\textbf{ Allconv}} \\  \hline
                        \multirow{5}{0.06\linewidth}{{\textbf{ Texture}}}
                        & Softmax score \cite{hendrycks2016baseline} & 83.29 & 73.34 & 92.89 & 86.04 & 70.90 & 91.99 \\
                        & Energy score (ours) & 79.41 & 76.28 & 93.63 & 81.30 & 76.47 & 93.50 \\
                        & ODIN \cite{liang2018enhancing} & 79.27 & 73.45 & 92.75 & 77.48 & 77.49 & 93.87 \\%(T=10/1000, noise=0.0038)
                        & Mahalanobis \cite{lee2018simple} & 39.39 & 90.57 & 97.74 & 42.64 & 87.02 & 96.41 \\
                        & OE \cite{hendrycks2018deep} & 61.11 & 84.56 & 96.19 & 71.16 & 79.47 & 94.71\\
                        & Energy fine-tuning (ours) & 57.01 & 87.40 & 96.95 & 59.26 & 86.46 & 96.77\\
                        \hline
                        % ----------- SVHN -----------------
                        \multirow{5}{0.06\linewidth}{{\textbf{ SVHN}}}
                        & Softmax score \cite{hendrycks2016baseline}
                        & 84.59 & 71.44 & 92.93 & 83.28 & 73.68 & 93.84\\
                        & Energy score (ours) & 85.82 & 73.99 & 93.65 & 76.33 & 86.15 & 97.15\\
                        & ODIN \cite{liang2018enhancing} & 84.66 & 67.26 & 91.38 & 60.93 & 88.34 & 97.46\\%(T=10/1000, noise=0.0038)
                        & Mahalanobis \cite{lee2018simple} & 57.52 & 86.01 & 96.68 & 21.23 & 95.28 & 98.91\\
                        & OE \cite{hendrycks2018deep} & 65.91 & 86.66 & 97.09 & 71.72 & 86.62 & 97.18\\
                        & Energy fine-tuning (ours) & 28.97 & 95.40 & 99.05 & 51.80 & 92.52 & 98.51\\
                        \hline
                        % ----------- Places -----------------
                        \multirow{5}{0.06\linewidth}{{\textbf{ Places365}}}
                        & Softmax score \cite{hendrycks2016baseline} & 82.84 & 73.78 & 93.29 & 82.21 & 74.98 & 93.79\\
                        & Energy score (ours) & 80.56 & 75.44 & 93.45 & 78.14 & 78.92 & 94.64\\
                        & ODIN \cite{liang2018enhancing} & 87.88 & 71.63 & 92.56 & 79.22 & 78.46 & 94.52\\%(T=10/1000, noise=0.0038)
                        &  Mahalanobis \cite{lee2018simple} & 88.83 & 67.87 & 90.71 & 95.32 & 57.12 & 86.97\\
                        & OE \cite{hendrycks2018deep} & 57.92 & 85.78 & 96.56 & 63.09 & 83.77 & 96.03\\
                        & Energy fine-tuning (ours) & 51.23 & 89.71 & 97.63 & 54.97 & 88.61 & 97.35\\
                        \hline
                        % ----------- LSUN-C -----------------
                        \multirow{5}{0.06\linewidth}{{\textbf{ LSUN-C}}}
                        & Softmax score \cite{hendrycks2016baseline} & 66.54 & 83.79 & 96.35 & 59.28 & 85.86 & 96.74\\
                        & Energy score (ours) & 35.32 & 93.53 & 98.62 & 23.00 & 95.73 & 99.07\\
                        & ODIN \cite{liang2018enhancing} & 55.55 & 87.73 & 97.22 & 18.13 & 96.59 & 99.28 \\%(T=10/1000, noise=0.0038)
                        & Mahalanobis \cite{lee2018simple} & 91.18 & 69.69 & 92.27 & 71.95 & 67.86 & 90.35\\
                        & OE \cite{hendrycks2018deep} & 21.92 & 95.81 & 99.08 & 24.10 & 94.56 & 98.71\\
                        & Energy fine-tuning (ours) & 16.04 & 96.97 & 99.34 & 18.50 & 96.64 & 99.28\\
                        \hline
                        % ----------- LSUN-R -----------------
                        \multirow{5}{0.06\linewidth}{{\textbf{ LSUN Resize}}}
                        & Softmax score \cite{hendrycks2016baseline} & 82.42 & 75.38 & 94.06 & 88.97 & 61.69 & 89.11\\
                        & Energy score (ours) & 79.47 & 79.23 & 94.96 & 77.37 & 73.64 & 92.72\\
                        & ODIN \cite{liang2018enhancing}& 71.96 & 81.82 & 95.65 & 72.15 & 75.87 & 93.44 \\%(T=10/1000, noise=0.0038)
                        &  Mahalanobis \cite{lee2018simple} & 21.23 & 96.00 & 99.13 & 83.70 & 74.64 & 93.67\\
                        & OE \cite{hendrycks2018deep} & 69.36 & 79.71 & 94.92 & 81.89 & 66.04 & 90.51\\
                        & Energy fine-tuning (ours)& 64.83 & 81.95 & 95.25 & 75.26 & 76.64 & 94.08\\
                        \hline
                        % ----------- iSUN -----------------
                        \multirow{5}{0.06\linewidth}{{\textbf{iSUN}}}
                        & Softmax score \cite{hendrycks2016baseline} & 82.80 & 75.46 & 94.06 & 88.06 & 62.53 & 89.27\\
                        & Energy score (ours) & 81.04 & 78.91 & 94.91 & 77.06 & 74.28 & 92.83\\
                        & ODIN \cite{liang2018enhancing} & 68.51 & 82.69 & 95.80 & 72.90 & 76.30 & 93.53 \\%(T=10/1000, noise=0.0038)
                        &  Mahalanobis \cite{lee2018simple} & 26.10 & 94.58 & 98.72 & 81.45 & 75.09 & 93.56\\
                        & OE \cite{hendrycks2018deep} & 72.39 & 78.61 & 94.58 & 82.18 & 65.83 & 90.21\\
                        & Energy fine-tuning (ours) & 67.23 & 79.36 & 94.37 & 74.08 & 76.77 & 93.99\\
                        %& EG fine-tuning $E_F,T=10$ (ours) \\
                        \bottomrule
                \end{tabular}
        \end{adjustbox}
        \vspace{-0.2cm}
        \caption[]{\small OOD Detection performance of CIFAR-100 as in-distribution for each specific dataset.  The Mahalanobis scores are calculated from the features of the second-to-last layer. %For ODIN, we set $T=1000$ and $\eta=0.0028$ for CIFAR-100\@. 
        }
        \label{tab:cifar100-results}
\end{table*}




% -------------------- WRN dense ----------------------

% \begin{table*}[]
%         \begin{adjustbox}{width=\columnwidth,center}
%                 \begin{tabular}{ll|ccc|ccc}
%                         \toprule
%                         \multirow{4}{0.08\linewidth}{$\mathcal{D}_{\text{in}}^{\text{test}}$} &  \multirow{4}{0.06\linewidth}{\textbf{Dataset $\mathcal{D}_{\text{out}}^{\text{test}}$}}  &\textbf{FPR}  &  \textbf{AUROC}  & \textbf{AUPR}  &\textbf{FPR}  & \textbf{AUROC}    &\textbf{AUPR}   \\
%                  & &  $\textbf{(95\% TPR)}$ & $\textbf{}$  & & $\textbf{(95\% TPR)}$ & $\textbf{}$  \\
%                         & & $\downarrow$ & $\uparrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\uparrow$ \\ \cline{3-8}
%                         & & \multicolumn{3}{c|}{\textbf{WRN}} & \multicolumn{3}{c}{\textbf{ DenseNet}} \\  \hline
%                         \multirow{9}{0.06\linewidth}{{\textbf{Texture}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 59.28 & 88.50 & 97.16 & 59.76 & 88.49 & 97.26\\
%                         & Energy score (ours) & 52.79 & 85.22 & 95.41 & 58.61 & 84.91 & 95.30\\
%                         & ODIN \cite{liang2018enhancing} & 49.12 & 84.97 & 95.28 & 57.07 & 81.53 & 93.95 \\%(T=10, noise=0.0004/0.0024)
%                         & Mahalanobis \cite{lee2018simple} & 15.00 & 97.33 & 99.41 & 19.84 & 94.29 & 98.46 \\
%                         & OE \cite{hendrycks2018deep} & 12.94 & 97.73 & 99.52 & 10.04 & 98.04 & 99.58\\
%                         & Energy fine-tuning (ours) & 5.34 & 98.56 & 99.68 & 5.67 & 98.15 & 99.45 \\
%                         \hline
%                         %------------------------SVHN----------------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{SVHN}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 48.49 & 91.89 & 98.27 & 59.17 & 89.92 & 97.86\\
%                         & Energy score (ours) & 35.59 & 90.96 & 97.64 & 47.57 & 90.94 & 98.03\\
%                         & ODIN \cite{liang2018enhancing} & 33.55 & 91.96 & 98.00 & 50.50 & 89.84 & 97.74\\
%                         & Mahalanobis \cite{lee2018simple} & 12.89 & 97.62 & 99.47 & 18.26 & 95.71 & 98.98 \\
%                         & OE \cite{hendrycks2018deep} & 4.36 & 98.63 & 99.74 & 3.55 & 99.07 & 99.82\\
%                         & Energy fine-tuning (ours) & 1.04 & 99.41 & 99.89 & 1.33 & 99.54 & 99.91 \\
%                         \hline
%                         % ----------------------- Places365 -------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{ Places365}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 59.48 & 88.20 & 97.10 & 59.00 & 88.87 & 97.39\\
%                         & Energy score (ours) & 40.14 & 89.89 & 97.30 & 45.59 & 90.14 & 97.60\\
%                         & ODIN \cite{liang2018enhancing} & 57.40 & 84.49 & 95.82 & 47.55 & 89.11 & 97.32\\
%                         & Mahalanobis \cite{lee2018simple} & 68.57 & 84.61 & 96.20 & 84.56 & 66.72 & 90.63 \\
%                         & OE \cite{hendrycks2018deep} & 19.07 & 96.16 & 99.06 & 13.42 & 96.86 & 99.22\\
%                         & Energy fine-tuning (ours) & 9.00 & 97.48 & 99.35 & 9.26 & 97.19 & 99.29 \\
%                         \hline
%                         % ----------------------- LSUN-C -----------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{ LSUN-C}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 30.80 & 95.65 & 99.13 & 38.53 & 94.89 & 99.00\\
%                         & Energy score (ours) & 8.26 & 98.35 & 99.66 & 7.87 & 98.31 & 99.66\\
%                         & ODIN \cite{liang2018enhancing} & 15.52 & 97.04 & 99.33 & 11.40 & 97.91 & 99.56 \\
%                         &  Mahalanobis \cite{lee2018simple} & 39.22 & 94.15 & 98.81 & 61.22 & 82.31 & 95.65 \\
%                         & OE \cite{hendrycks2018deep} & 2.89 & 99.49 & 99.90 & 1.21 & 99.68 & 99.94\\
%                         & Energy fine-tuning (ours) & 1.67 & 99.32 & 99.86 & 0.84 & 99.03 & 99.82 \\
%                         \hline
%                         % --------------------LSUN-R --------------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{ LSUN Resize}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 52.15 & 91.37 & 98.12 & 32.92  & 95.47 & 99.11\\
%                         & Energy score (ours) & 27.58 & 94.24 & 98.67 & 8.09 & 98.36 & 99.67\\
%                         & ODIN \cite{liang2018enhancing} & 26.62 & 94.57 & 98.77 & 3.90 & 99.21 & 99.84\\
%                         & Mahalanobis \cite{lee2018simple} & 42.62 & 93.23 & 98.60 & 11.84 & 97.34 & 99.38 \\
%                         & OE \cite{hendrycks2018deep} & 5.59 & 98.94 & 99.79 & 1.87 & 99.45 & 99.89\\
%                         & Energy fine-tuning (ours) & 1.25 & 99.39 & 99.88 & 0.59 & 99.59 & 99.92 \\
%                         \hline
%                         % -------------iSUN --------------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{iSUN}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 56.03 & 89.83 & 97.74 & 36.50 & 94.86 & 98.99\\
%                         & Energy score (ours) & 33.68 & 92.62 & 98.27 & 10.98 & 97.96 & 99.59\\
%                         & ODIN \cite{liang2018enhancing} & 32.05 & 93.50 & 98.54 & 6.01 & 98.87 & 99.76 \\
%                         & Mahalanobis \cite{lee2018simple} & 44.18 & 92.66 & 98.45 & 15.55 & 96.50 & 99.15 \\
%                         & OE \cite{hendrycks2018deep} & 6.32 & 98.85 & 99.77 & 1.90 & 99.45 & 99.89\\
%                         & Energy fine-tuning (ours) & 1.60 & 99.33 & 99.87 & 0.90 & 99.57 & 99.91 \\
%                         %& EG fine-tuning $E_F,T=10$ (ours) \\
%                         \bottomrule
%                 \end{tabular}
%         \end{adjustbox}
%         \vspace{-0.2cm}
%         \caption[]{\small OOD Detection performance of CIFAR-10 as in-distribution for each OOD test dataset.
%         The Mahalanobis score is calculated using the features of the second-to-last layer. \JDO{Bold the best scores.}}
%         \label{tab:cifar10-results}
% \end{table*}



% \begin{table*}[]
%         \begin{adjustbox}{width=\columnwidth,center}
%                 \begin{tabular}{ll|ccc|ccc}
%                         \toprule
%                         \multirow{4}{0.08\linewidth}{$\mathcal{D}_{\text{in}}^{\text{test}}$} &  \multirow{4}{0.06\linewidth}{\textbf{Dataset $\mathcal{D}_{\text{out}}^{\text{test}}$}}  &\textbf{FPR}  &  \textbf{ AUROC}  & \textbf{ AUPR}  &\textbf{FPR}  & \textbf{AUROC}  &\textbf{AUPR}   \\
%                  & &  $\textbf{(95\% TPR)}$ & $\textbf{}$  & & $\textbf{(95\% TPR)}$ & $\textbf{}$  \\
%                         & & $\downarrow$ & $\uparrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\uparrow$ \\ \cline{3-8}
%                         & & \multicolumn{3}{c|}{\textbf{WRN}} & \multicolumn{3}{c}{\textbf{ DenseNet}} \\  \hline
%                         \multirow{9}{0.06\linewidth}{{\textbf{ Texture}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 83.29 & 73.34 & 92.89 & 81.23 & 72.78 & 92.16 \\
%                         & Energy score (ours) & 79.41 & 76.28 & 93.63 & 78.80 & 73.94 & 91.06 \\
%                         & ODIN \cite{liang2018enhancing} & 79.27 & 73.45 & 92.75 & 77.20 & 75.55 & 92.28\\%(T=10/1000, noise=0.0038)
%                         & \S Mahalanobis \cite{lee2018simple} & 39.39 & 90.57 & 97.74 & 36.29 & 87.70 & 96.15 \\
%                         & OE \cite{hendrycks2018deep} & 61.11 & 84.56 & 96.19 & 70.03 & 81.39 & 95.16\\
%                         & Energy fine-tuning (ours) & 57.01 & 87.40 & 96.95 & 65.18 & 83.36 & 95.36 \\
%                         \hline
%                         % ----------- SVHN -----------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{ SVHN}}}
%                         & Softmax score \cite{hendrycks2016baseline}
%                         & 84.59 & 71.44 & 92.93 & 73.58 & 82.95 & 96.27\\
%                         & Energy score (ours) & 85.82 & 73.99 & 93.65 & 65.81 & 87.84 & 97.41\\
%                         & ODIN \cite{liang2018enhancing} & 84.66 & 67.26 & 91.38 & 51.84 & 90.21 & 97.88\\%(T=10/1000, noise=0.0038)
%                         & Mahalanobis \cite{lee2018simple} & 57.52 & 86.01 & 96.68 & 49.51 & 87.36 & 96.83 \\
%                         & OE \cite{hendrycks2018deep} & 65.91 & 86.66 & 97.09 & 52.69 & 91.33 & 98.21\\
%                         & Energy fine-tuning (ours) & 28.97 & 95.40 & 99.05 & 34.86 & 93.50 & 98.67 \\
%                         \hline
%                         % ----------- Places -----------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{ Places365}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 82.84 & 73.78 & 93.29 & 80.87  & 75.88 & 93.95 \\
%                         & Energy score (ours) & 80.56 & 75.44 & 93.45 & 79.23 & 78.00 & 94.41 \\
%                         & ODIN \cite{liang2018enhancing} & 87.88 & 71.63 & 92.56 & 76.19 & 79.15 & 94.63\\%(T=10/1000, noise=0.0038)
%                         &  Mahalanobis \cite{lee2018simple} & 88.83 & 67.87 & 90.71 & 95.69 & 54.91 & 86.27 \\
%                         & OE \cite{hendrycks2018deep} & 57.92 & 85.78 & 96.56 & 61.08 & 85.81 & 96.60\\
%                         & Energy fine-tuning (ours) & 51.23 & 89.71 & 97.63 & 61.80 & 84.80 & 96.18 \\
%                         \hline
%                         % ----------- LSUN-C -----------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{ LSUN-C}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 66.54 & 83.79 & 96.35 & 60.50 & 85.24 & 96.61\\
%                         & Energy score (ours) & 35.32 & 93.53 & 98.62 & 20.82 & 96.24 & 99.17\\
%                         & ODIN \cite{liang2018enhancing} & 55.55 & 87.73 & 97.22 & 17.36 & 96.69 & 99.29\\%(T=10/1000, noise=0.0038)
%                         & Mahalanobis \cite{lee2018simple} & 91.18 & 69.69 & 92.27 & 41.97 & 94.77 & 99.01 \\
%                         & OE \cite{hendrycks2018deep} & 21.92 & 95.81 & 99.08 & 20.86 & 96.02 & 99.12\\
%                         & Energy fine-tuning (ours) & 16.04 & 96.97 & 99.34 & 24.45 & 94.95 & 98.98 \\
%                         \hline
%                         % ----------- LSUN-R -----------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{ LSUN Resize}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 82.42 & 75.38 & 94.06 & 83.56 & 70.81 & 92.68\\
%                         & Energy score (ours) & 79.47 & 79.23 & 94.96 & 76.86 & 79.58 & 95.10\\
%                         & ODIN \cite{liang2018enhancing}& 71.96 & 81.82 & 95.65 & 60.10 & 85.48 & 96.57\\%(T=10/1000, noise=0.0038)
%                         &  Mahalanobis \cite{lee2018simple} & 21.23 & 96.00 & 99.13 & 13.31 & 97.19 & 99.39 \\
%                         & OE \cite{hendrycks2018deep} & 69.36 & 79.71 & 94.92 & 78.56 & 78.37 & 94.90 \\
%                         & Energy fine-tuning (ours)& 64.83 & 81.95 & 95.25 & 64.07 & 90.95 & 98.07 \\
%                         \hline
%                         % ----------- iSUN -----------------
%                         \multirow{9}{0.06\linewidth}{{\textbf{iSUN}}}
%                         & Softmax score \cite{hendrycks2016baseline} & 82.80 & 75.46 & 94.06 & 85.27 & 69.44 & 92.15\\
%                         & Energy score (ours) & 81.04 & 78.91 & 94.91 & 80.78 & 77.45 & 94.50\\
%                         & ODIN \cite{liang2018enhancing} & 68.51 & 82.69 & 95.80 & 63.65 & 84.11 & 96.20\\%(T=10/1000, noise=0.0038)
%                         &  Mahalanobis \cite{lee2018simple} & 26.10 & 94.58 & 98.72 & 16.77 & 96.28 & 99.12 \\
%                         & OE \cite{hendrycks2018deep} & 72.39 & 78.61 & 94.58 & 79.39 & 76.91 & 94.38\\
%                         & Energy fine-tuning (ours) & 67.23 & 79.36 & 94.37 & 68.44 & 89.14 & 97.50 \\
%                         %& EG fine-tuning $E_F,T=10$ (ours) \\
%                         \bottomrule
%                 \end{tabular}
%         \end{adjustbox}
%         \vspace{-0.2cm}
%         \caption[]{\small OOD Detection performance of CIFAR-100 as in-distribution for each specific dataset.  The Mahalanobis scores are calculated from the features of the second-to-last layer. %For ODIN, we set $T=1000$ and $\eta=0.0028$ for CIFAR-100\@. 
%         \JDO{Bold the best scores.}}
%         \label{tab:cifar100-results}
% \end{table*}

==> tex/discussion.tex <==
\section{Discussion}


==> tex/gda.tex <==
\section{Energy Score Under Gaussian Discriminative Analysis}
\label{A: GDA}
Similar to Mahalanobis score~\cite{lee2018simple}, our method assumes the neurons $f(x)$ of the second last hidden layer distributes as Multi-Dimensional Gaussian, the basic assumption of Gaussian Discriminant Analysis (GDA). Moreover, Linear Discriminant Analysis (LDA) is applied and thus all classes share the same covariant matrix $\Sigma$ for the Multi-Dimensional Gaussian. Given the class mean is $\mathbf{\mu_c}$, $P(f(\*x)|y=c)=\mathcal{N}(f(\*x)-\mathbf{\mu_c}, \mathbf{\Sigma})$. If we set the priors $P(y=c) = \pi_c$, the posterior can be written as
\begin{align*}
    P(y=c|\*x)
    &=\frac{P(y=c)P(f(\*x)|y=c)}{\sum_{c^{'}} P(y=c^{'}) P(f(\*x)|y=c^{'})} \\
    &=\frac{P(y=c)e^{-(f(\*x)-\mathbf{\mu}_c)^T\Sigma^{-1}(f(\*x)-\mathbf{\mu}_c)}}{\sum_{c^{'}} P(y=c^{'}) e^{-(f(\*x)-\mathbf{\mu}_{c^{'}})^T\Sigma^{-1}(f(\*x)-\mathbf{\mu}_{c^{'}})}} \\
    &=\frac{e^{-(f(\*x)-\mathbf{\mu}_c)^T\Sigma^{-1}(f(\*x)-\mathbf{\mu}_c)+\text{ln}(\pi_c)}}{\sum_{c^{'}} e^{-(f(\*x)-\mathbf{\mu}_{c^{'}})^T\Sigma^{-1}(f(\*x)-\mathbf{\mu}_{c^{'}})+\text{ln}(\pi_{c^{'}})}} \\
\end{align*}
Compared the above equation to Equ~\ref{equ:softmax7}, we have 
\begin{align*}
    E_U(\*x; f)
    &= \sum_c^C[(f(\*x)-\mathbf{\mu}_c)^T\Sigma^{-1}(f(\*x)-\mathbf{\mu}_c)+\text{ln}(\pi_c)]P(y=c|\*x)\\
\end{align*}
Given a model $f$ estimated on data $\*x\sim P_\mathbf{X}$, if $\*x_{in}$ is an in-distribution sample where $f$ can map it sufficiently close to one of class mean $\mu_{c_{'}}$, and if $\*x_{out}$ is an out-distribution sample where $f$ can map it far away from any of the class means $\mu_c$, then $E_U(x_{in}; f) \le E_U(x_{out}; f)$. 

For simplicity, we set the number of classes $C=2$ and the class means are $\mu_0$ and $\mu_1$. We use the 
property of co-variance matrix $\Sigma$. $\Sigma$ is 
symmetric positive definite if $x_i$ is independent.  $\Sigma^{-1}$ exists, and $\Sigma^{-1}$ is also symmetric and positive definite. Then
\begin{align}
    E_U(\*x_{in}; f)
    &= [(f(\*x_{in})-\mathbf{\mu}_0)^T\Sigma^{-1}(f(\*x_{in})-\mathbf{\mu}_0)+\text{ln}(\pi_0)]P(y=0|\*x_{in}) \nonumber\\
    &+[(f(\*x_{in})-\mathbf{\mu}_1)^T\Sigma^{-1}(f(\*x_{in})-\mathbf{\mu}_1)+\text{ln}(\pi_1)]P(y=1|\*x_{in}) \nonumber\\
    &= P(y|\* x_{in}) (f(\*x_{in}) - \mu_0)^T \Sigma ^{-1} (f(\*x_{in}) - \mu_0) \nonumber \\
    &+ P(y= 1| \*x_{in}) (f(\*x_{in})^T \Sigma^{-1}f(\*x_{in}) - 2f(\*x_{in})^T\Sigma ^{-1} \mu_1  \nonumber\\
    &+ 2 f(\*x_{in})^T \Sigma ^{-1} \mu_0 + \mu_1^T\Sigma^{-1} \mu_1 - \mu_0^T \Sigma ^{-1} \mu_0)
    +\text{ln}(\pi_0)P(y=0|\*x_{in})+\text{ln}(\pi_1)P(y=1|\*x_{in}) \nonumber\\
    &=  P(y=0|\* x_{in}) (f(\*x_{in}) - \mu_0)^T \Sigma ^{-1} (f(\*x_{in}) - \mu_0) \nonumber \\ 
    &+ P(y=1|X_{in}) [(f(\*x_{in})-\mu_1+\mu_0)^T \Sigma ^{-1} (f(\*x_{in})-\mu_1+\mu_0) \nonumber \\
    &+ 2(\mu_0 + 0.5\mu_1)^T \Sigma ^{-1} (\mu_0 + 0.5\mu_1) - 0.5 \mu_1 ^T \Sigma^{-1} \mu_1] 
    +\text{ln}(\pi_0)P(y=0|\*x_{in})+\text{ln}(\pi_1)P(y=1|\*x_{in}) \nonumber \\
\label{eq: left}
\end{align}
On the other hand,
\begin{align}
    E_U(\*x_{out}; f)
    &= [(f(\*x_{out})-\mathbf{\mu}_0)^T\Sigma^{-1}(f(\*x_{out})-\mathbf{\mu}_0)+\text{ln}(\pi_0)]P(y=0|\*x_{out}) \nonumber \\
    &+[(f(\*x_{out})-\mathbf{\mu}_1)^T\Sigma^{-1}(f(\*x_{out})-\mathbf{\mu}_1)+\text{ln}(\pi_1)]P(y=1|\*x_{out}) \nonumber \\
    &= P(y|\*x_{out}) (f(\*x_{out}) -a )^T \Sigma ^{-1} (f(\*x_{out}) -a ) \label{eq:eq8}\\ 
    &+ P(y= 0| \*x_{out}) P(y=1 | y \cap \*x_{out} )
    (\mu_0 - \mu_1) ^T \Sigma ^{-1} (\mu_0 - \mu_1) \label{eq: eq9} \\
    &+ \text{ln}(\pi_0)P(y=0|\*x_{out}) + \text{ln}(\pi_1)P(y=1|\*x_{out}) \label{eq:eq10} \\
    \label{eq:right}
\end{align}

where $a = P(y=0 | y \cap x_{out}) \mu_0 + p(y=1 | y \cap x_{out}) \mu_1$. 
As long as the network maps out-distribution sample $f(x_{out})$ sufficiently far away from any of the class means, $E_U(\*x_{in}; f) < K < E_U(\*x_{out}; f)$.\SL{How  is this derived?} \XY{using "almost everywhere" ? }

Consider minima of formula (~\ref{eq: eq9}) + (~\ref{eq:eq10}) appears at either $P(y=0|\*x_{out}) =0$ or $P(y=1|\*x_{out}) =0$, so the lower bound of  $E_U(\*x_{out}; f)$ is formula (~\ref{eq:eq8}) + $min( \text{ln}(\pi_0),  \text{ln}(\pi_1))$. 

The upper bound of formula (~\ref{eq: left}), 




\para{Lemma}: for vector $x$ and $y$, if $||x|| > ||y||$, and with a symmetric and positive definite matrix $\Sigma$, $x^T \Sigma x $ is also bigger than $y^T\Sigma y$. 

Proof: Since $\Sigma$ is positive definite and symmetric, $\Sigma = Q \Lambda Q^T$, where $\Lambda$ is a diagonal matrix with each element $\lambda_{ii} >0$, and $Q$ is a orthogonal matrix. 

Thus $x^T\Sigma X = x^TQ\Lambda Q^{T}x$; As we know
$||QA|| = \sqrt{(QA, QA)} = \sqrt{(Q^TQA, A)} = ||A||$ with $Q$ is orthogonal.
Thus if $||x||>||y||$ then $||Qx||>||Qy||$. Since $\Lambda$ is a diagonal matrix with each element greater than 0, we can easily see that $x^T\Sigma x > y^t \Sigma y$. 
%from https://en.wikipedia.org/wiki/Eigendecomposition_of_a_matrix
% The posterior of the Softmax score of class $c$ given the trained weights $\*w_c$ and $b_c$ and input $\*x$ is:
% \begin{align*}
%     P(y=c|\*x)
%     &=\frac{e^{\*w_c^T f(\*x)+b_c}}{\sum_{c^{'}} e^{\*w_c^T f(\*x)+b_{c^{'}}}} \\
% \end{align*}

% We will illustrate our ideas of energy indicator through two simple Gaussian distributions with different means and standard deviation: N($\mu_1, \sigma_1^2$) and N($\mu_2, \sigma_2^2$). We form a prior distribution $p(x)$ of two classes and assign probability of choosing the first class as
% \begin{align*}
%     a = \frac{\frac{1}{\sqrt{2\sigma_1^2}}exp(-(x-\mu_1)^2 / (2\sigma_1^2))}{\frac{1}{\sqrt{2\sigma_1^2}}exp(-(x-\mu_1)^2 / (2\sigma_1^2)) + \frac{1}{\sqrt{2\sigma_2^2}}exp(-(x-\mu_2)^2 / (2\sigma_2^2))}
% \end{align*}
% Thus, this classifier should have probability distribution $(a, 1-a)$ of choosing the first class and second class. If we sample from $p(x)$ and train a Softmax regression classifier $q(x)$ with features $x$ and $x^2$ as input, the weights of the best classifier will be exactly the same as $p$, because we form our prior as exact the same form as Softmax regression. Thus, the energy $U$ of the empirical distribution $q(x)=p(x)$ should be
% \begin{align*}
%      U = \frac{a(x-\mu_1)^2}{2\sigma_1^2} + \frac{(1-a)(x-\mu_2)^2}{2\sigma_2^2}
% \end{align*}
% The formula $U$ we derived clearly shows that when $x_0$ is sampled from another distribution and is substantially different from $x_1$ that is sampled from the prior $p(x)$, it is likely that the corresponding $U(x_0)$ is higher than the $U(x_1)$.

==> tex/prelim.tex <==
\section{Preliminaries}
% In this section, we will introduce the OOD detection problem and existing approaches. 

% \subsection{Out-of-distribution Detection}
\label{subsec:ood-techs}
Out-of-distribution detection can be formulated as a canonical binary classification problem. Suppose the image space is $\mathcal{X}  \subset \mathbb{R}^n$ and the label class space is $\mathcal{Y}=\{1,2,\cdots,K \}$. Assume that a neural network $f(\theta)$ is trained on a dataset $\mathcal{D}_{\text{in}}^{\text{train}}$ drawn from a data distribution $P_{\bm{X},Y}$ defined on $\mathcal{X} \times \mathcal{Y}$. Let $P_{\bm{X}}$ denote the marginal distribution of $P_{\bm{X},Y}$. We refer to $P_{\bm{X}}$  as  \textbf{in-distribution}. An OOD classifier $G:\mathcal{X}\mapsto \{0,1\}$ is built to distinguish whether an input $\*x$ is from $P_{\bm{X}}$ (give it label $1$) or not (give it label $0$). 
% Here, we have an assumption that inputs are either drawn from $P_{\bm{X}}$ or distributions that are sufficiently different from $P_{\bm{X}}$. Thus, the conceptual objective of OOD detection can be viewed as:
% \begin{align*}
% 	\min_G \quad \mathbb{E}_{\*x\sim P_{\bm{X}}} \mathbb{I}[G(x)=0] 
% 	+ \sum_{\mathcal{O}_{\bm{X}} \in \mathscr{D}_{\bm{X}}} \mathbb{E}_{\*x\sim \mathcal{O}_{\bm{X}}}  \mathbb{I}[G(x)=1],
% \end{align*}
% where $\mathscr{D}_{\bm{X}}$ is the family of all distributions defined on the image space $\mathcal{X}$ that are sufficiently different from $P_{\bm{X}}$. In practice, it can be intractable to directly optimize this objective due to lack of prior knowledge on $\mathscr{D}_{\bm{X}}$. We will describe a few surrogate methods to this objective in Section~\ref{subsec:ood-techs}.

In testing, the detector  $G$ is evaluated on natural images drawn from a mixture distribution ${\mathcal{M}}_{\bm{X}\times Z}$ defined on $\mathcal{X}\times\{0,1\}$, where the conditional probability distributions ${\mathcal{M}_{\bm{X}|Z=0}=P_{\bm{X}}}$ and ${\mathcal{M}}_{\bm{X}|Z=1}=Q_{\bm{X}}$.  $Q_{\bm{\bm{X}}}$ is a distribution different from $P_{\bm{\bm{X}}}$, which we refer to as  \textbf{out-distribution}. 

% Usually, $G$ is evaluated on an in-distribution test set $\mathcal{D}_{\text{in}}^{\text{test}}$ drawn from $P_{\bm{X}}$ and an out-of-distribution test set $\mathcal{D}_{\text{out}}^{\text{test}}$ drawn from $Q_{\bm{\bm{X}}}$.

The detector $G(\*x)$ in practice can be used as an auxiliary classifier to filter out-of-distribution examples. Once an input $\*x$ is verified to be in-distribution example, one can simply run it through the neural network $f(\theta)$ to classify it.

% \subsection{Existing Softmax-based Approaches}
% \label{subsec:ood-techs}

% Recently, several approaches have been proposed to detect OOD examples based on different notions of confidence scores. These methods typically rely on the softmax score produced by the neural networks.

% \textbf{Maximum Softmax Probability (MSP).} Maximum Softmax Probability method is as a common baseline for OOD detection \cite{hendrycks2016baseline}. Given an input image $\*x$ and a pre-trained neural network $f(\cdot)$, the softmax output of the classifier is computed by 
% $$F(\*x)=\frac{e^{f_i(\*x)}}{\sum_{j=1}^{K} e^{f_j(\*x)}}.$$

% A threshold-based detector  $G(\*x)$ relies on the confidence score $S(\*x;f) = \max_i F_i(\*x)$ to make prediction as follows
% \begin{align}
% G_{\text{MSP}}(\*x; \gamma, f) = 
% \begin{cases} 
% 1 & \quad \text{if } S(\*x;f) > \gamma \\
% 0 & \quad \text{if } S(\*x;f) \leq \gamma 
% \end{cases}
% \end{align} 
% where $\gamma$ is the confidence threshold. 
% %This method works under the assumption that a neural network produces high confidence predictions  for  in-distribution samples and low confidence on the out-of-distribution samples. 

% \textbf{ODIN.}  The original softmax confidence scores used in \cite{hendrycks2016baseline} can be over-confident.  ODIN~\cite{liang2017enhancing} leverages this insight and improves the MSP baseline using the calibrated confidence score instead~\cite{guo2017calibration}. Specifically, the calibrated confidence score is computed by 
% $$S(\*x;T,f)=\max_i \frac{e^{f_i(\*x)/T}}{\sum_{j=1}^{K} e^{f_j(\*x)/T}},$$
% where $T \in \mathbb{R}^+$ is the temperature scaling parameter. In addition, ODIN applies small noise perturbation to the inputs 
% \begin{equation}
% \label{eq:perturbation}\tilde{{\*x}}={{\*x}}-\eta \cdot \text{sign}(-\nabla_{{{\*x}}}\log S({{\*x}};T, f)),
% \end{equation}
% where the parameter $\eta$ is the perturbation magnitude. 

% By combining the two components together, ODIN detector $G_{\text{ODIN}}$ is given by
% \begin{align}
% G_{\text{ODIN}}(\*x; T, \eta, \gamma, f) = 
% \begin{cases} 
% 1 & \quad \text{if } S(\tilde{\*x};T,f) > \gamma \\
% 0 & \quad \text{if } S(\tilde{\*x};T,f)  \leq \gamma 
% \end{cases}
% \end{align} 
% In real applications, it may be difficult to know the out-of-distribution one will encounter in advance. The hyperparameters of $T$ and $\eta$ can be tuned instead on a random noise data such as Gaussian or uniform distribution, without requiring prior knowledge of OOD dataset. 

% \textbf{Outlier Exposure (OE).} Outlier Exposure \cite{hendrycks2018deep} makes use of a large, unlabeled auxiliary dataset $\mathcal{D}_{\text{out}}^{\text{OE}}$ to improve out-of-distribution detection. A new classifier, $F_\text{OE}$, parameterized by $\theta$, is trained using the following objective
% \begin{align*}
% \min_\theta & \quad \mathbb{E}_{(\*x,y)\sim \mathcal{D}_{\text{in}}^{\text{train}}}[-\log {F_y}(\*x)] \\
% & + \lambda \cdot \mathbb{E}_{\*x \sim \mathcal{D}^{\text{OE}}_{\text{out}}}[L_{\text{CE}}({F}(\*x), \mathcal{U}_K
% )], 
% \end{align*}
% where $F(\cdot)$ is softmax output of the classification model trained on $P_{\bm{X},Y}$, and $\mathcal{U}_K$ is the uniform distribution over $K$ classes. The cross-entropy loss $L_{\text{CE}}(z, y)=- \sum_{i=1}^K y_i \log z_i$. This objective regularizes the model $F$ to produce more conservative  predictions (uncertainties) on the out-of-distribution samples.  The classifier $F_{\text{OE}}$ can be combined with downstream OOD detection methods (such as MSP). The outlier exposure (OE) detector can be constructed as $G_{\text{MSP}}(\*x; \gamma, F_{\text{OE}})$. 


==> tex/table_adv.tex <==
% \begin{table}[t]
% \caption{Adversarial benchmark results for Mahalanobis and energy gap for unknown attack on ResNet. Results with and without fine-tuning of TinyImages80m are shown. While other methods trained their regression through FGSM, our model is not exposed to any of the attack. \label{table:M_adv}}
% %\begin{center}
% \begin{tabular}{|c|ccccc|}
% \hline
% \centering
% \multirow{2}{*}{Dataset}
% &\multicolumn{5}{c}{AUROC for ResNet} \\
% &\multicolumn{1}{c}{Score}
% &\multicolumn{1}{c}{FGSM}
% &\multicolumn{1}{c}{BIM}
% &\multicolumn{1}{c}{DeepFool}
% &\multicolumn{1}{c}{CW} \\
% \hline
% \multirow{5}{*}{CIFAR10}
%     & \multicolumn{1}{l}{KD+PU~\cite{feinman2017detecting}}   & 83.51 & 16.16 & 76.80 & 56.30 \\
%     & \multicolumn{1}{l}{LID~\cite{ma2018characterizing}}     & 99.69 & 95.38 & 71.86 & 77.53 \\
%     & \multicolumn{1}{l}{Mahalanobis~\cite{lee2018simple}} & \textbf{99.94} & \textbf{98.91} & 78.06 & \textbf{93.90} \\
%     & \multicolumn{1}{l}{EG $F$ w/o fine-tuning (ours)}  & 88.75 & *94.90 & \textbf{89.07} & 61.36 \\
%     & \multicolumn{1}{l}{EG $F$ fine-tuning (ours)}  & 91.80 & *- & 89.50 & 68.57 \\
%     & \multicolumn{1}{l}{EG $U$ w/o fine-tuning (ours)}  & 88.72 & *94.89 & 89.19 & 61.38 \\
%     & \multicolumn{1}{l}{EG $U$ fine-tuning (ours)} & 91.48 & *- & 88.49 & 71.76 \\
% \hline
% \multirow{7}{*}{CIFAR100}
%     & \multicolumn{1}{l}{KD+PU~\cite{feinman2017detecting}}   & 89.90 & 68.85 & 57.78 & 73.72 \\
%     & \multicolumn{1}{l}{LID~\cite{ma2018characterizing}}     & 98.73 & 55.82 & 63.15 & 75.03 \\
%     & \multicolumn{1}{l}{Mahalanobis~\cite{lee2018simple}} & \textbf{99.77} & \textbf{96.38} & 81.95 & \textbf{90.96} \\
%     & \multicolumn{1}{l}{EG $F$ w/o fine-tuning (ours)}  & 90.80 & *91.57 & \textbf{86.82} & 79.92 \\
%     & \multicolumn{1}{l}{EG $F$ fine-tuning (ours)}  & 92.59 & *- & 84.97 & 76.93 \\
%     & \multicolumn{1}{l}{EG $U$ w/o fine-tuning (ours)}  & 90.96 & *91.49 & 86.95 & 79.87 \\
%     & \multicolumn{1}{l}{EG $U$ fine-tuning (ours)}  & 90.81 & *- & 84.99 & 78.56 \\
% \hline
% \multirow{5}{*}{SVHN}
%     & \multicolumn{1}{l}{KD+PU~\cite{feinman2017detecting}}   & 82.67 & 43.21 & 84.30 & 67.85 \\
%     & \multicolumn{1}{l}{LID~\cite{ma2018characterizing}}     & 97.86 & 84.88 & 67.28 & 76.58 \\
%     & \multicolumn{1}{l}{Mahalanobis~\cite{lee2018simple}} & \textbf{99.62} & \textbf{95.39} & 72.20 & \textbf{86.73} \\
%     & \multicolumn{1}{l}{EG $F$ w/o fine-tuning (ours)}  & 87.21 & *64.74 & \textbf{93.25} & 77.04 \\
%     & \multicolumn{1}{l}{EG $F$ fine-tuning (ours)}  & 98.72 & *- & 93.04 & 91.31 \\
%     & \multicolumn{1}{l}{EG $U$ w/o fine-tuning (ours)} & 87.22 & *64.66 & 93.35 & 77.09 \\
%     & \multicolumn{1}{l}{EG $U$ fine-tuning (ours)}  & 98.77 & *- & 92.98 & 91.27 \\
% \hline
% \end{tabular}
% %\end{center}
% \end{table}

\begin{table*}[t]
	\begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{ll|cccc}
			\toprule
			\multirow{1}{0.08\linewidth}{$\mathcal{D}_{\text{in}}^{\text{test}}$} &  \multirow{1}{0.06\linewidth}{\textbf{Method}}  &\bf{FGSM}  & \bf{BIM}  & \bf{DeepFool}  & \bf{CW}   \\
			\hline 
			\multirow{6}{0.06\linewidth}{{{\bf CIFAR-10}}}
			& $\S$KD+PU~\cite{feinman2017detecting} & 83.51 & 16.16 & 76.80 & 56.30 \\
			& $\S$LID~\cite{ma2018characterizing} & 99.69 & 95.38 & 71.86 & 77.53 \\ 
			& $\S$Mahalanobis~\cite{lee2018simple} & 99.94 & 98.91 & 78.06 & 93.90 \\
			& EG $E_U$ score (ours) & 87.38 & $\dag$95.09 & 88.00 & 61.04\\
			& EG $E_F$ score (ours) & 87.42 & $\dag$95.10 & 87.86 & 61.02 \\
			& Mahalanobis \cite{lee2018simple} & 99.98 & 98.91 & 90.53 & 91.05  \\
			& EG fine-tuning $E_U,T=1$ (ours) &  & - &\\
			& EG fine-tuning $E_U,T>1$ (ours) & & - &\\
			& EG fine-tuning $E_U$+ODIN (ours) & & - &\\
			& EG fine-tuning $E_F,T=1$ (ours) & & - &\\
			& EG fine-tuning $E_F,T>1$ (ours) & & - &\\
			& EG fine-tuning+$E_F$+ODIN (ours) & & - &\\
			\hline
			\multirow{6}{0.06\linewidth}{{\bf CIFAR-100}}
			& $\S$KD+PU~\cite{feinman2017detecting}   & 89.90 & 68.85 & 57.78 & 73.72 \\
			& $\S$LID~\cite{ma2018characterizing}     & 98.73 & 55.82 & 63.15 & 75.03 \\
			& $\S$Mahalanobis~\cite{lee2018simple} & 99.77 & 96.38 & 81.95 & 90.96 \\
			& EG $E_U$ score (ours) & 90.42 & $\dag$91.71 & 86.17 & 79.42 \\
			& EG $E_F$ score (ours) & 90.25 & $\dag$91.79 & 86.04 & 79.47 \\
			& Mahalanobis \cite{lee2018simple} & 99.37 & 86.87 & 77.50 & 77.04 \\
		    & EG fine-tuning $E_U,T=1$ (ours) & & - &\\
			& EG fine-tuning $E_U,T>1$ (ours) & & - &\\
			& EG fine-tuning $E_U$+ODIN (ours) & & - &\\
			& EG fine-tuning $E_F,T=1$ (ours) & & - &\\
			& EG fine-tuning $E_F,T>1$ (ours) & & - &\\
			& EG fine-tuning+$E_F$+ODIN (ours) & & - &\\
			\hline
			\multirow{6}{0.06\linewidth}{{\bf SVHN}}
			& $\S$KD+PU~\cite{feinman2017detecting} & 82.67 & 43.21 & 84.30 & 67.85 \\
			& $\S$LID~\cite{ma2018characterizing} & 97.86 & 84.88 & 67.28 & 76.58 \\
			& $\S$Mahalanobis~\cite{lee2018simple} & 99.62 & 95.39 & 72.20 & 86.73 \\
			& EG $E_U$ score (ours) & 87.12 & $\dag$64.70 & 93.05 & 77.05 \\
			& EG $E_F$ score (ours) & 87.11 & $\dag$64.79 & 92.93 & 77.00 \\
			& Mahalanobis \cite{lee2018simple} & 97.64 & 91.81 & 91.75 & 86.43\\
		    & EG fine-tuning $E_U,T=1$ (ours) & & - &\\
			& EG fine-tuning $E_U,T>1$ (ours) & & - &\\
			& EG fine-tuning $E_U$+ODIN (ours) & & - &\\
			& EG fine-tuning $E_F,T=1$ (ours) & & - &\\
			& EG fine-tuning $E_F,T>1$ (ours) & & - &\\
			& EG fine-tuning+$E_F$+ODIN (ours) & & - &\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\vspace{-0.2cm}
	\caption[]{\small Distinguishing clean and adversarial test set data for image classification. $\dag$ indicates in-distribution examples have higher energy than adversarial examples and no energy fine-tuning is performed. $\S$ indicates methods that train their regression models and tune hyperparameters based on FGSM while other attack types are unknown. The results on DenseNet can be found in Appendix~\ref{sec:complete-experimental-results}.}
	\label{tab:adv_main-results}
\end{table*}

==> tex/theory_method.tex <==
\section{Background:  Energy-based Models}
\label{sec:background}

% An energy model assigns low energy values for observed data, whereas unseen examples lead to configurations with higher energy~\cite{lecun2006tutorial}.


% \subsection{Energy Functions}\label{sec:energy_def}

% The concept of internal energy and free energy are well-known in statistical mechanics~\cite{balescu1975equilibrium}


 %Assume the {energy} is statistically distributed across $K$ output units of a neural network. %Each unit $f(\*x; \theta)$ has an energy $E_i$ and is associated with a probability $p_i$.


% \SL{TODO: this part needs major editing. Add more context about EBM. Add another subsection about connection to softmax - bring logit shift to the picture upfront.}
% \JDO{One of the things I find frustrating about machine learning papers is gratuituous math. You don't use $\theta$ for anything interesting in this entire section. If you removed all uses of $\theta$ you would lose no meaning at all. Why do you use $\theta$?}

The essence of the energy-based model (EBM)~\cite{lecun2006tutorial} is to build a function $E(\*x): \mathbb{R}^D \rightarrow \mathbb{R}$ that maps each
point $\*x$ of an input space to a single, non-probabilistic scalar called the \emph{energy}. %A data point takes low energy value when it has a high probability of occurrence.
% \WL{I would phrase this sentence as Lower energy has higher probability of occurrence. Or I would comment out the next sentence, since it is not very essential in this section.  }
% The idea of EBM
% is rooted in physics, with the intuition
%  that observed data represent low-energy configurations, whereas unseen examples have higher energy.
%  While energies are  measured in arbitrary unit, it is possible to turn a collection of arbitrary energies into a collection of probability scores whose sum (or integral) is 1 through Gibbs distribution:
 A collection of energy values could be turned into a probability density $p(\*x)$ through the Gibbs distribution:
\begin{equation}\label{eq:gibbs}
    p(y \mid \*x) = \frac{e^{-E(\*x,y)/T}}{\int_{y'} e^{-E(\*x, y')/T}}
    = \frac{e^{-E(\*x,y)/T}}{e^{-E(\*x)/T}},
\end{equation}
% \begin{equation}
%     p(\*x) = \frac{e^{-E(\*x)/T}}{\int_{\*x}e^{-E(\*x)/T}} = \frac{e^{-E(\*x)/T}}{Z}
% \end{equation}
 where the denominator $\int_{y'} e^{-E(\*x, y')/T}$ is called the partition function, which marginalizes over $y$, and $T$ is the temperature parameter. The \emph{Helmholtz free energy} $E(\*x)$ of a given data point $\*x \in \mathbb{R}^D$ can be expressed as the negative of the log partition function:
 \begin{equation}
     E(\*x) = -T \cdot \log \int_{y'} e^{-E(\*x, y')/T}
 \end{equation}

\para{Energy Function} The energy-based model has an inherent connection with modern  machine learning, especially discriminative models.
% As shown in~\cite{ grathwohl2019your}, one can re-interpret a neural classifier to define a density function $p(\*x)$ over $\*x \in \mathbb{R}^D$.
To see this, we consider a discriminative neural classifier $f(\*x): \mathbb{R}^D\rightarrow \mathbb{R}^K$, which maps an input $\*x\in \mathbb{R}^D$ to $K$ real-valued numbers known as logits. These logits are used to derive a categorical distribution using the softmax function:
\begin{equation}\label{eq:softmax}
    p(y \mid \*x) = \frac{e^{f_y(\*x)/T}}{\sum_{i}^K e^{f_{i}(\*x)/T}},
\end{equation}
where $f_y(\*x)$ indicates the $y^\text{th}$ index of $f(\*x)$, i.e., the logit corresponding to the $y^\text{th}$ class label.
% can be characterized by
% this framework: for each $\*x$ in the training set, the energy of the pair ($\*x$, y) takes lower values when
% $y$ is the correct label, and higher otherwise.

% \begin{align}
%     p(y \mid \*x) &=\frac{e^{f_y(\*x)/T}/Z}{\sum_{i}^K e^{f_{i}(\*x)/T}/Z} \\
%     &=\frac{p(\*x,y)}{p(\*x)}.
% \end{align}
% The equation above suggests that one can obtain the density function $p(\*x)$ without changing the parameterization of the neural network $f(\*x)$:
% \begin{equation}
%     p(\*x) = \frac{\sum_{i}^K e^{f_{i}(\*x)/T}}{Z}
% \end{equation}
By connecting Eq.~\ref{eq:gibbs} and Eq.~\ref{eq:softmax}, we can define an energy for a given input $(\*x, y)$ as $E(\*x,y) = -f_y(\*x)$. More importantly, without changing the parameterization of the neural network $f(\*x)$, we can express the free energy function $E(\*x;f)$ over $\*x\in \mathbb{R}^D$ in terms of the denominator of the softmax activation:
\begin{align}\label{eq:energy_softmax}
  E(\*x;f)=- T\cdot \text{log}\sum_i^K e^{f_i(\*x)/T}.
\end{align}

% \subsection{JEM}
% In this subsection, we summarize and highlight the methodological distinctions between our work and JEM~\cite{grathwohl2019your}, as both are related to energy-based models.

% First, the idea of using the energy score for OOD detection is novel and theoretically motivated. JEM~\cite{grathwohl2019your} used likelihood score $\log p(\*x)$ from \textbf{generative} modeling or softmax score; we instead derive the energy score from a \textbf{pure discriminative} model. % \hl{motivated by the mathematical connection  between the data distribution $p(x)$ and energy.}.
% We showed both mathematical insights in Section~\ref{sec:energy-inference} and empirical success that energy is better than softmax score---which was not presented in JEM.

% Secondly, JEM's optimization is intractable as it requires estimating the normalized densities w.r.t.\ all inputs $\*x$. Specifically, JEM  estimates the joint distribution $\log p_\theta(\*x, y) = \log p_\theta(\*x) + \log p_\theta(y|\*x)$. The first term maximizes the likelihood from a generative modeling perspective, which requires estimating normalized densities. As pointed out by Grathwohl et al.~\cite{grathwohl2019your} in the limitations (Sec.\ 6), \emph{``Energy based models can be very challenging to work with. Since normalized likelihoods cannot be
% computed, it can be hard to verify that learning is taking place at all~\ldots{} Furthermore, the gradient estimators we use to train JEM are quite unstable and are
% prone to diverging if the sampling and optimization parameters are not tuned correctly.''} In contrast, ours is easy to optimize using standard SGD, and doesn't involve proper normalization.

% Thirdly, JEM only uses in-distribution data. Our training objective~(\ref{eq:fine-tune-obj}) leverages auxiliary outlier data and explicitly enlarges the energy gap, which is also different from Outlier Exposure\@.


\section{Energy-based Out-of-distribution Detection}
\label{sec:method}

We propose a unified framework using an energy score for OOD detection, where the differences of energies between in- and out-of-distribution allow effective differentiation.
The energy score mitigates a critical problem of softmax confidence with arbitrarily high values for OOD examples~\cite{hein2019relu}. In the following, we first describe using energy as an OOD score for pre-trained models, and the connection between the energy and softmax scores~(Section \ref{sec:energy-inference}). We then describe how to use  energy as a trainable cost function for model fine-tuning~(Section \ref{sec:energy-ft}).

\subsection{Energy as Inference-time OOD Score}\label{sec:energy-inference}

Out-of-distribution detection is a binary classification problem that relies on a score to differentiate between in- and out-of-distribution examples. A scoring function should produce values that are  distinguishable between in- and out-of-distribution.
% A common approach is to use the softmax confidence score $\max_y p(y|\*x)$ and classify examples with low scores as out-of-distribution. However, a critical problem with softmax is that it can produce arbitrarily high confidence score for OOD inputs~\cite{hein2019relu}.
A natural choice is to use the density function of the data $p(\*x)$ and consider examples
with low likelihood to be OOD\@.
% However, previous research showed that density function estimated through deep generative models cannot be reliably used for OOD detection~\cite{nalisnick2018deep}.
While it is possible to obtain the density function for a discriminative model by resorting to the energy-based model~\cite{lecun2006tutorial, grathwohl2019your}:
\begin{align}\label{eq:density}
    p(\*x) = \frac{e^{-E(\*x;f)/T}}{\int_{\*x}e^{-E(\*x;f)/T}},
\end{align}
% \WL{Do we need the following definition? We define the normalized densities (partition function) for $p(x)$ as $Z=\int_{\*x}e^{-E(\*x)/T}$ over $\*x \in \mathbb{R}^D$.}
the normalized densities $Z=\int_{\*x}e^{-E(\*x;f)/T}$ (with respect to $\*x$) can be intractable to compute or even reliably estimate over the input space.

To mitigate the challenge, our key observation is that the absence of the normalization does not affect the OOD detection at all. A data point with a higher probability of occurrence is equivalent to having lower energy. To see this, we can take the logarithm of both sides of Eq.~\ref{eq:density},
\begin{align*}
    % e^{-E(\*x;f)/T} &\propto p(\*x) \\
    \log p(\*x) & = -E(\*x;f) / T - \hspace{-2.9ex}\underbrace{\log Z.}_{\text{\normalfont constant for all  $\*x$}}
    % \implies -E(\*x;f) &\propto \log p(\* x)
\end{align*}
% \begin{align} I just leave the original version if you don't think proportional makes sense.
%     p(\*x) = \frac{e^{-E(\*x)/T}}{\int_{\*x}e^{-E(\*x)/T}} = \frac{\sum_i^K e^{f_i(\*x)/T}}{Z},
% \end{align}
The equation above suggests that $-E(\*x;f)$ is in fact linearly aligned with the log likelihood function, which is desirable for OOD detection. Examples with higher energies (lower likelihood) are considered as OOD inputs.
%When we choose the free energy defined in Eq.~\ref{eq:energy_softmax} as $E(\*x)$, we can simply use the unnormalized energy score for OOD detection, where examples with higher energies are considered as OOD inputs.
Specifically, we propose using the energy function $E(\*x;f)$ in~Eq.~\ref{eq:energy_softmax} for OOD detection:
\begin{align}
G(\*x; \tau, f) =
\begin{cases}
0 & \quad \text{if } -E(\*x;f) \leq \tau, \\
1 & \quad \text{if } -E(\*x;f) > \tau,
\end{cases}
\end{align}
where $\tau$ is the energy threshold. In practice, we choose the threshold using in-distribution data so that a high fraction of inputs are correctly classified by the OOD detector $G(\*x)$.
% \JDO{See: previous comment about gratuitous math. I don't see that you use $G$ in any significant way in the rest of this paper.}
% The energy function $E(\*x;f)$ can be either internal energy $E_U$ or free energy $E_F$. \JDO{The reader right now is wondering ``which one do I choose and why'' and that better be answered pretty soon, and the ``why'' is really important here.}
Here we use negative energy scores, $-E(\*x;f)$, to align with the conventional definition where positive (in-distribution) samples have higher scores. The energy score is non-probabilistic in nature, which can be conveniently calculated via the \texttt{logsumexp} operator. Unlike JEM~\cite{grathwohl2019your}, our method does not require estimating the density  $Z$ explicitly, as $Z$ is sample-independent and does not affect the overall energy score distribution.
% \JDO{Please check previous sentence for accuracy.}
% Then during inference time, a given new example $\*x$ with negative energy lower than the threshold $\tau$ is classified as OOD (with label 0).

\begin{figure}
\begin{center}
\subfigure[ softmax scores 1.0 vs.\ 0.99]{\includegraphics[width=60mm]{fig/dist.pdf}}
\subfigure[  negative energy scores: 11.19 vs.\ 7.11]{\includegraphics[width=60mm]{fig/logit.pdf}}
% \subfigure[]{\includegraphics[width=60mm]{fig/msp_cor_f_wro.pdf}}
% \subfigure[]{\includegraphics[width=60mm]{fig/msp_wro_f_cor.pdf}}
\caption{\small (a) Softmax and (b) logit outputs of two samples calculated on a CIFAR-10 pre-trained WideResNet. The out-of-distribution sample is from SVHN\@. For (a), the softmax confidence scores are 1.0 and 0.99 for the in- and out-of-distribution examples. In contrast, the energy scores calculated from logit are $E(\*x_{\text{in}})=-11.19$, $E(\*x_{\text{out}})=-7.11$. While softmax confidence scores are almost identical for in- and out-distribution samples, energy scores provide more meaningful information with which to differentiate them. %\SL{Can we change the color to be gray and blue that matches Figure 2?}
  % (c) Logits and probabilities of an OOD sample where MSP detection is correct but $E_F$ detection is wrong. (d) Logits and probabilities of an OOD sample where MSP detection is wrong but $E_F$ detection is correct.
 % \JDO{This is really confusing. The caption+figure labels say you're comparing softmax and logits. The figures say you're comparing MSP and energy. You have to be consistent here. And it looks to me like MSP is doing a great job~\ldots\ in-distribution samples are completely separate from OOD samples.}
\label{fig:dist_ex_msp_vs_f} %\SL{Anyway we can update the color to be the same as in Fig 3?}
}
\vspace{-0.5cm}
\end{center}
\end{figure}

\para{Energy Score vs.\ Softmax  Score}\label{sec:discussion} Our method can be used as a simple and effective replacement for the softmax confidence score~\cite{hendrycks2016baseline} for any pre-trained neural network.
% We first provide  conceptual reasoning, which highlights an important difference between energy score and softmax confidence score $\max_y p(y \mid \*x)$.
% % \WL{Shall we rename softmax score, softmax confidence score or MSP to MSP only to avoid interchangeable terms, which are potentially confusing?}
% In particular, we consider a simple example, where the logit of one input $\*x_1$ is $f(\*x_1)$, and the logit of another input $\*x_2$ is $f(\*x_1)$ minus an arbitrary scalar $a$.
% % \JDO{I edited the previous sentence, please check that it's right. I didn't like the idea that the second input ``shifted'' the first input, because I thought they are computed independently.}
% Notice that the softmax confidence scores remain the same between $\*x_1$ and $\*x_2$ since:
% \begin{align}
% \max_y p(y \mid \*x_1) & = \max_y \frac{e^{f_y(\*x_1)/T}}{\sum_{i}^K e^{f_{i}(\*x_1)/T}}\\
% & = \max_y \frac{e^{(f_y(\*x_1)-a)/T}}{\sum_{i}^K e^{(f_y(\*x_1)-a)/T}} = \max_y p(y \mid \*x_2)
% \end{align}
% % In contrast, the energy scores derived from the logits, $E(\*x_1)$ and $E(\*x_2)$, are different and better distinguish the two inputs. Thus, a key insight is that energy score uses extra degree of freedom hidden within the logits to differentiate in- and out-of-distribution examples: %Energy score in some sense breaks the softmax score's symmetry of ``constant shift'':
% % \begin{align}
% %     -T \cdot \text{log}\sum_i^K e^{f_i(\*x_1)/T} \ne -T \cdot \text{log}\sum_i^K e^{(f_i(\*x_1)-a)/T}.
% % \end{align}
% The problem of softmax confidence score is that two different inputs can generate significantly different logits, but they can end up with similar softmax confidence score. In contrast, the energy scores derived from the logits, $E(\*x_1)$ and $E(\*x_2)$, are different and better distinguish the two inputs:
% \begin{align}
%     -T \cdot \text{log}\sum_i^K e^{f_i(\*x_1)/T} \ne -T \cdot \text{log}\sum_i^K e^{(f_i(\*x_1)-a)/T}.
% \end{align}
To see this, we first derive a mathematical connection between the energy score and the softmax confidence score:
% The detailed derivation is provided in Appendix~\ref{A: connection}, where we show:
\begin{align*}
\max_y p(y \mid \*x)
    &= \max_y \frac{e^{f_y(\*x)}}{\sum_{i} e^{f_{i}(\*x)}}
    = \frac{e^{ f^{\text{max} }(\*x)}}{\sum_{i} e^{f_{i}(\*x)}}\\
    &= \frac{1}{\sum_i e^{f_i(\*x)-f^{\text{max} }(\*x)}} \\
    \implies \log \max_y p(y \mid \*x) &= E(\*x; f(\*x)-f^{\text{max}}(\*x)) = E(\*x; f)+f^{\text{max}}(\*x),
\end{align*}
when $T=1$. This reveals that the log of the softmax confidence score is in fact equivalent to a special case of the free energy score, where all the logits are shifted by their maximum logit value. Since $f^{\text{max}}(\*x)$ tends to be higher and $E(\*x; f)$ tends to be lower for in-distribution data, the shifting results in a biased scoring function that is no longer proportional to the probability density $p(\*x)$ for $\*x \in\mathbb{R}^D$:
\begin{align*}
    \log \max_y p(y \mid \*x) &=  -\log p(\*x) + \hspace{-2.8ex}\underbrace{f^{\text{max}}(\*x) - \log Z}_{\text{\normalfont Not constant. Larger for in-dist $\*x$}} \\
    & \not\propto -\log p(\*x).
\end{align*}
As a result, unlike the energy score, which is well aligned with density $p(\*x)$, the softmax confidence score is less able to reliably distinguish in- and out-of-distribution examples.
% In fact, the term $f^{\text{max}}(\*x)$ is large while $-\log p(\*x)$ being small for in-distribution data, and therefore making softmax confidence score less able to reliably distinguish in- and out-of-distribution.
To illustrate with a real example, Figure~\ref{fig:dist_ex_msp_vs_f} shows one example from the SVHN dataset (OOD) and another example from the in-distribution data CIFAR-10\@. While their softmax confidence scores are almost identical (1.0 vs 0.99), the negative energy scores are more distinguishable (11.19 vs.\ 7.11).  Thus, working in the original logit space (energy score) instead of the shifted logit space (softmax score) yields more useful information for each sample.
% , and in some sense, breaks the softmax's symmetry of ``constant shift''. \JDO{Again this is a new term that hasn't been introduced before. Maybe your readers all know this term already. I don't.}
We show in our experimental results in Section~\ref{sec:results} that energy score is a superior metric for OOD detection than the softmax score. %We provide more discussion on the connection in Section~\ref{sec:discussion}.
%The shifting of logits loses meaningful information that otherwise energy function exploits to distinguish between in- and out-of-distribution examples.%A key problem with softmax confidence score is that two different inputs can generate significantly different logits, but they can end up with similar softmax confidence score. For example, when shifting the logits $f(\*x)$ by a constant scalar $a$, the softmax remains the same. In contrast, the energy scores derived from the logits are different and better distinguish the two inputs.


% \JDO{So I think this following argument needs to go higher in the paper. This next sentence is in fact the problem that you want to solve. It would be better to present the problem up front, then talk about how you solve it.}
% A critical problem of softmax is that two different sets of logits can be mapped to very similar softmax confidence scores.
% While shifting the logits $f(\*x)$ by an arbitrary scalar does not change the softmax confidence score, the shifting can result in different energy scores. Energy function therefore
% \WL{preserves the information within logits and produce more distinguishable scores for inputs that have high softmax confidence scores (overconfidence issue).}
% exploits the extra degree of freedom within the logits and produces more distinguishable scores.


% \JDO{I would tend to structure the argument like this:
%   \begin{enumerate}
%     \item We currently use softmax as our metric for distinguishing ID and OOD\@.
%     \item Softmax takes into account these things (x, y, z) but does not take into account these things (a, b, c).
%     \begin{itemize}
%       \item I don't know if the following is true or not, but it seems to me that softmax is playing two roles here: one is classifying the inputs into categories and one is classifying the inputs as OOD vs.\ ID\@.
%     \end{itemize}
%     \item These are good decisions for softmax for its traditional role. But they are bad decisions if what you're trying to do is classify OOD vs.\ ID\@.
%     \item Why? They ignore this really important thing. When you ignore this thing, here's what happens. We think the decision needs to take into account this thing.
%     \item It turns out that a similar problem has been addressed in the statistical mechanics community. They need to solve the following problem (describe problem), and they solve it (briefly) in the following way. It turns out our problem and their problem are actually very similar, and thus the inspiration for our energy function comes from their formulation of \ldots
%   \end{enumerate}
% }

% \WL{I leave two versions here. John's above and the new below (with the numbers updated), as I cant decide the issues above are solved.}
% A critical problem of softmax is that two different sets of logits can be mapped to very similar softmax confidence scores. Unlike softmax confidence scores, energy function exploits the extra degree of freedom within the logits and produces scores that are more distinguishable.
% To illustrate with a real example, Figure~\ref{fig:dist_ex_msp_vs_f} shows one example from the SVHN dataset (OOD) and another example from the in-distribution data CIFAR-10\@. While their softmax confidence scores are almost identical (1.0 vs. 0.99), the negative energy scores relying on logits are more distinguishable (11.19 vs. 7.11).  Thus, working in the original logit space (energy score) instead of the shifted logit space (softmax score) yields more useful information for each sample samples, and in some sense, breaks the softmax's symmetry of ``constant shift''.  We  show experimental results in Section~\ref{sec:results} that energy score works considerably better than the softmax score for OOD detection. %We provide more discussion on the connection in Section~\ref{sec:discussion}.


% Similarly, a detector $G_F(\*x)$ relies on the internal energy $E_F(\*x;f)$ can be defined as
% \begin{align}
% G_{F}(\*x; \gamma, f) =
% \begin{cases}
% 0 & \quad \text{if } -E_F(\*x;f) \leq \tau \\
% 1 & \quad \text{if } -E_F(\*x;f) > \tau
% \end{cases}
% \end{align}
% where $\tau$ is the energy threshold.

\begin{figure}
\begin{center}
%\includegraphics[width=70mm]{fig/c10_fpr.png}
%\includegraphics[width=70mm]{fig/c10_error.png}
\subfigure[FPR95: 48.49~\label{fig:MSP_demo}]{\includegraphics[width=67mm]{fig/MSP.pdf}}
\subfigure[FPR95: 35.59~\label{fig:U_demo}]{\includegraphics[width=67mm]{fig/F.pdf}}
\subfigure[FPR95: 4.36]{\includegraphics[width=67mm]{fig/OE.pdf}}
\subfigure[FPR95: 1.04]{\includegraphics[width=67mm]{fig/OE_F.pdf}}
\caption{\small (a \& b) Distribution of softmax scores vs.\ energy scores from pre-trained WideResNet. We contrast the score distribution from fine-tuned models using Outlier Exposure~\cite{hendrycks2018deep} (c) and our energy-bounded learning (d).
 We use negative energy scores for (b \& d) to align with the convention that positive (in-distribution) samples have higher scores.
 Using energy score leads to an overall smoother distribution (b \& d), and is less susceptible to the spiky distribution that softmax exhibits for in-distribution data (a \& c). \label{fig:dist}
 \vspace{-0.5cm}
%\SL{Update this to be free energy. Let's just say "Energy score (pretrained)" and "Energy score (fine-tuning)" for plot title}
}
\end{center}
\end{figure}
% When training, the model tries to increase the logit that corresponds to the correct label while decrease the the other logits in order to minimize the cross entropy between the ground truth distribution and network predicted distribution. Thus, the logit of the correct class should be higher than the wrong classes logits and so as its probability; Equ~\ref{equ:softmax7} for $U$ only has $logit_{i=\text{label}}*p_{i=\text{label}}$ dominated. Based on the same reasoning, the model lowers the $U_{i \in training}$ of each sample $i$ in the training set. We believe $U$ could be a very simple and yet effective indicator of OOD dataset: $U$ could be smaller for the training (and test) set than other OOD test sets, which the model is not directly trained on.

% If this OOD indicator is utilized, the case when the maximum logit equals to 0 should be avoided, because $logit_{i=\text{label}}*p_{i=\text{label}}$ will not dominate. A common technique should be avoided that shifts the logits by its maximum logits in order to avoid overflow of exponential. Otherwise, this case is not common since there is generally no constraint on the logit values in deep learning objective.


% We did not notice significant differences in experiments between $F$ and $U$ for OOD detection. Yet, one of the previous methods~\cite{hendrycks2018deep} has $F$ as part of their optimization objective. We will discuss the connection in next subsection.
%------------------------------------------%
\subsection{Energy-bounded Learning for OOD Detection}\label{sec:energy-ft}

While energy score can be useful for a pre-trained neural network, the energy gap between in- and out-of-distribution might not always be optimal for differentiation. Therefore, we also propose an energy-bounded learning objective, where the neural network  is fine-tuned to \emph{explicitly} create an energy gap by assigning lower energies to the in-distribution data, and higher energies to the OOD data.
% \JDO{I \emph{think} this is trained simultaneously with the rest of the network, although it's not quite clear to me if you're trying to maximize the gap or simply train so $G$ is accurate. I think based on the discussion below it's the former.}
The learning process allows greater flexibility in contrastively shaping the energy surface, resulting in more distinguishable in- and out-of-distribution data.
% Can we enlarge the energy gap between the in-data and out-data so as to improve its performance of OOD detection? Our idea is to fine-tune the classification model by enforcing a constant energy gap between training data and outliers. We propose an energy-bounded learning objective, leveraging an auxiliary unlabeled dataset $\mathcal{D}_{\text{out}}^{\text{OE}}$ as in~\cite{hendrycks2018deep}. The training objective encourages the model to contrastively assign low energy for in-distribution data, and higher energy for outlier samples.
Specifically, our energy-based classifier is trained using the following objective:
\begin{align}\label{eq:fine-tune-obj}
\min_\theta & \quad \mathbb{E}_{(\*x,y)\sim \mathcal{D}_{\text{in}}^{\text{train}}}[-\log {F_y}(\*x)] + \lambda \cdot L_\text{energy}
\end{align}
where $F(\*x)$ is the softmax output of the classification model and $\mathcal{D}_{\text{in}}^{\text{train}}$ is the in-distribution training data. The overall training objective combines the standard cross-entropy loss, along with a regularization loss defined in terms of energy:
% \begin{align}
%   L_\text{energy} & = \mathbb{E}_{(\*x_\text{in},y)\sim \mathcal{D}_{\text{in}}^{\text{train}}} \min(0, m_{\text{in}}-E(\*x_\text{in})) \\
%   & + \mathbb{E}_{\*x_\text{out}\sim \mathcal{D}_{\text{out}}^{\text{OE}}} \max(0, m_{\text{out}}-E(\*x_\text{out}))
% \end{align}
% MSE+OE: The benefit is $m_{in}$ and $m_{out}$ are in the gradient now.
\begin{align}
  L_\text{energy} & = \mathbb{E}_{(\*x_\text{in},y)\sim \mathcal{D}_{\text{in}}^{\text{train}}} (\max(0, E(\*x_\text{in})-m_{\text{in}}))^2 \\
  & + \mathbb{E}_{\*x_\text{out}\sim \mathcal{D}_{\text{out}}^{\text{train}}} (\max(0, m_{\text{out}}-E(\*x_\text{out})))^2
\end{align}
where $\mathcal{D}_{\text{out}}^{\text{train}}$ is the unlabeled auxiliary OOD training data~\cite{torralba200880}.
In particular, we regularize the energy using two squared hinge loss terms\footnote{We also explored using a hinge loss such as $\max(0, E(\*x_\text{in})-E(\*x_\text{out})+m) $ through a single constant margin parameter $m$. While the difference between $E(\*x_\text{in})$ and $E(\*x_\text{out})$ can be stable, their values do not stabilize. Optimization is more flexible and the training process is more stable with two separate hinge loss terms.} with separate margin hyperparameters $m_\text{in}$ and $m_\text{out}$.
In one term, the model penalizes in-distribution samples that produce energy higher than the specified margin parameter $m_\text{in}$. Similarly, in another term, the model penalizes the out-of-distribution samples with energy lower than the margin parameter $m_\text{out}$.
% Since the model is agnostic to the true OOD test sets a priori, we leverage an auxiliary unlabeled dataset $\mathcal{D}_{\text{out}}^{\text{train}}$ as surrogate OOD training data~\cite{torralba200880}.
% $m_{\text{in}}$ and $m_{\text{out}}$ are two hyperparameters where $m_{\text{in}} < m_{\text{out}}$.
In other words, the loss function penalizes the samples with energy $E(\*x) \in [m_{\text{in}}, m_{\text{out}}]$.
Once the model is fine-tuned, the downstream OOD detection is similar to our description in Section~\ref{sec:energy-inference}.

%While the energy score can be interpreted from the likelihood view, the optimization processes of JEM~\cite{grathwohl2019your}  vs. ours are very different.
% $This term then encourages the free energy for in-data to be lower than $m_{\text{in}}$ and the free energy for out-data to be higher than $m_{\text{out}}$.


% We propose a fine-tuning objective of energy $L_{en}$ along with the original loss $L_{ori}$ for in-data, given that the network is able to access datasets other than its original training set. The total loss for fine-tuning is simply:
% \begin{equation*}
%   L_{tot} = L_{en}(x_{in}, x_{out}) + L_{ori}(x_{in})
% \end{equation*}
% where $x_{in}$ is an in-data sample and $x_{out}$ is an out-data sample. Out-data sample does not contribute to $L_ori$.

% Inspired by the objective of EB-GAN~\cite{zhao2019energy}, our propose the energy objective is (one sample version):
% \begin{equation*}
%   L_{en} = min(0, m_{in}-F(x_{in})) + max(0, m_{out}-F(x_{out}))
% \end{equation*}
% where $m_{in}$ is the upper bound of free energy for in-data, $m_{out}$ is the lower bound of free energy for out-data. They are hyperparameters to be tuned and most importantly, $m_{in} <= m_{out}$ based on our previous discussion. This loss penalizes the samples with free energy $F \in [m_{in}, m_{out}]$. This term then encourages the free energy for in-data to be lower than $m_{in}$ and the free energy for out-data to be higher than $m_{out}$. Moreover, our preliminary results show that the energy gap must be bounded; otherwise, this new objective keeps generating the gradient and worsens the classification performance.

% \para{Connection to Outlier Exposure Objective.} We draw comparison between our energy-based objective with outlier exposure (OE)~\cite{hendrycks2018deep}, where enforces the prediction for outlier samples to be close to uniform distribution. This ends up with an additional objective to the loss with cross entropy:
% \begin{align*}
%   L
%   &= KL(\mathbf{p} || \mathbf{q}) \\
%   &= -(\frac{1}{K}\sum_i^K f_i(x) - \text{logsumexp}(\mathbf{logit})) \\
%   &= \text{mean}(\mathbf{logit}) - E(x_\text{out})
% \end{align*}
% where $\mathbf{logit}$ is a prediction vector and $K$ is the number of classes. The last equation clearly shows the connection and difference between our proposed energy gap and outlier-exposure. Outlier-exposure always tries to encourage the free energy $E(x_\text{out})$ to be higher while decrease the mean of logits. While our method encourages $E(x_\text{out})$ to be higher as well, it sets energy bounds for both in-distribution data and outlier data, penalizing them only when those values are in the gap.

% \section{Theoretical Interpretation}
% Given a model $f$ estimated on data $x\sim P_\mathbf{X}$, we now express our OOD score as a subtraction between the negative log likelihood and free energy $E_F(\*x;f)$:
% \begin{align}
% S(\*x) = -\log p(\*x| f) - |E_F(\*x;f)|.
% \end{align}
% Notice that, since we use negative log-likelihood and  energy, the higher the score $S(\*x)$, the more OOD the input $\*x$ will be.

% Interestingly, $S$ can be interpreted as a likelihood-ratio test statistic. We can think of an energy model $\mathcal{M}_0$ as a universal model, adjusted for all possible inputs and general enough so that it assigns high energy value for any point off the data manifold. Considering the probabilistic model associated with the energy of the input, we have
% \begin{align}
%   p(\*x|\mathcal{M}_0) = 2^{-|E_F(\*x;f)|}.
% \end{align}

% Alternatively, a ‘simpler’ model $\mathcal{M}$ is trained targeting specific semantics or data type. With it, one aims to approximate the marginal likelihood (or model evidence) for $\*x\in \mathcal{X}$ , which integrates out all model
% parameters:
% \begin{align}
%   p(\*x|\mathcal{M}) = \int p(\*x| \theta, \mathcal{M})p(\theta|\mathcal{M}) d\theta
% \end{align}
% This integral is intractable, but we can approximate $p(\*x|\mathcal{M})$ under Gaussian Discriminative Analysis (GDA). Specifically, we define $K$ class-conditional multivariate Gaussian distributions with a tied covariance $\*\Sigma$:
% \begin{align}
%   p(\*x|y=k) & = \mathcal{N}(\*x| {\boldsymbol{\mu}}_k, \*\Sigma)\\
%   & = \frac{1}{\sqrt{(2\pi)^d |\*\Sigma|}}\exp(-\frac{(\*x-{\boldsymbol{\mu}}_k)^T \*\Sigma^{-1}(\*x-{\boldsymbol{\mu}}_k)}{2}),
% \end{align}
% where where ${\boldsymbol{\mu}}_k$ is the mean of multivariate Gaussian distribution of class $k \in \{1, ..., K\}$. The mean of the $k$-th class can be estimated using e Maximum Likelihood Estimation (MLE), or method of moments (MOM), for the mean of a Gaussian distirbution:
% \begin{align}
%   \mathbb{R}^d \in \hat{\boldsymbol{\mu}}_k = \frac{1}{n_k} \sum_{i=1}^n\*x_i\cdot \mathbb{I}(\mathcal{C}(\*x_i)=k),
% \end{align}
% where $\mathbb{I}(\cdot)$ is an indicator function. And the covariance matrix can be estimated by
% \begin{align}
%  \mathbb{R}^{d\times d} \in \*{\hat \Sigma} = \frac{1}{n} \sum_{k=1}^K\sum_{i=1}^n (\*x_i-\hat{\boldsymbol{\mu}}_k)(\*x_i-\hat{\boldsymbol{\mu}}_k)^T \mathbb{I}(\mathcal{C}(\*x_i)=k)
% \end{align}

% Based on a theoretical connection between GDA
% and the softmax classifier, the posterior distribution defined by the generative classifier under GDA
% with tied covariance is equivalent to the softmax classifier $f(\*x)$ (see proof in the appendix).

% Using the above induced class-conditional Gaussian distributions, the log likelihood can be defined using Mahalanobis distance between
% test sample $\*x$ and the closest class-conditional Gaussian distribution:
% \begin{align}
%  \text{Mahalanobis}(\*x)= \max_k - (\*x-\hat{\boldsymbol{\mu}}_k)^T \*{\hat\Sigma}^{-1}(\*x-\hat{\boldsymbol{\mu}}_k),
% \end{align}
% which also corresponds to measuring the log of the probability densities of the test sample.

% Choosing between one or another model is then reduced to a simple likelihood ratio
% \begin{align}
%   \log_2\frac{p(\mathcal{M}_0|\*x)}{p(\mathcal{M}|\*x)} & = \log_2\frac{p(\*x|\mathcal{M}_0)p(\mathcal{M}_0)}{p(\*x|\mathcal{M})p(\mathcal{M})}\\
%   & = \log_2\frac{p(\*x|\mathcal{M}_0)}{p(\*x|\mathcal{M})}
% \end{align}
% under uniform priors.
% This ratio is therefore reduced to
% \begin{align}
%   S(\*x) & = -\log_2 p(\*x|\mathcal{M}) + \log_2 p(\*x|\mathcal{M}_0) \\
%   & = -\text{Mahalanobis}(\*x) - |E_F(\*x;f)|
% \end{align}

